Community Needs and Assets: A Computational Analysis of Community Conversations

A community needs assessment is a tool used by non-profits and government agencies to quantify the strengths and issues of a community, allowing them to allocate their resources better. Such approaches are transitioning towards leveraging social media conversations to analyze the needs of communities and the assets already present within them. However, manual analysis of exponentially increasing social media conversations is challenging. There is a gap in the present literature in computationally analyzing how community members discuss the strengths and needs of the community. To address this gap, we introduce the task of identifying, extracting, and categorizing community needs and assets from conversational data using sophisticated natural language processing methods. To facilitate this task, we introduce the first dataset about community needs and assets consisting of 3,511 conversations from Reddit, annotated using crowdsourced workers. Using this dataset, we evaluate an utterance-level classification model compared to sentiment classification and a popular large language model (in a zero-shot setting), where we find that our model outperforms both baselines at an F1 score of 94% compared to 49% and 61% respectively. Furthermore, we observe through our study that conversations about needs have negative sentiments and emotions, while conversations about assets focus on location and entities. The dataset is available at https://github.com/towhidabsar/CommunityNeeds.

==> sections/8_checklist.tex <==
\section{Paper Checklist to be included in your paper}
\newcommand{\answerYes}[1]{\textcolor{blue}{#1}} 
\newcommand{\answerNo}[1]{\textcolor{teal}{#1}} 
\newcommand{\answerNA}[1]{\textcolor{gray}{#1}} 
\newcommand{\answerTODO}[1]{\textcolor{red}{#1}} 
\begin{enumerate}

\item For most authors...
\begin{enumerate}
    \item  Would answering this research question advance science without violating social contracts, such as violating privacy norms, perpetuating unfair profiling, exacerbating the socio-economic divide, or implying disrespect to societies or cultures?
    \answerYes{Yes}
  \item Do your main claims in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{Yes}
   \item Do you clarify how the proposed methodological approach is appropriate for the claims made? 
    \answerYes{Yes}
   \item Do you clarify what are possible artifacts in the data used, given population-specific distributions?
    \answerYes{Yes}
  \item Did you describe the limitations of your work?
    \answerYes{Yes}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Yes}
      \item Did you discuss any potential misuse of your work?
    \answerYes{Yes}
    \item Did you describe steps taken to prevent or mitigate potential negative outcomes of the research, such as data and model documentation, data anonymization, responsible release, access control, and the reproducibility of findings?
    \answerYes{Yes}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{Yes}
\end{enumerate}

% \item Additionally, if your study involves hypotheses testing...
% \begin{enumerate}
%   \item Did you clearly state the assumptions underlying all theoretical results?
%     \answerTODO{Answer}
%   \item Have you provided justifications for all theoretical results?
%     \answerTODO{Answer}
%   \item Did you discuss competing hypotheses or theories that might challenge or complement your theoretical results?
%     \answerTODO{Answer}
%   \item Have you considered alternative mechanisms or explanations that might account for the same outcomes observed in your study?
%     \answerTODO{Answer}
%   \item Did you address potential biases or limitations in your theoretical framework?
%     \answerTODO{Answer}
%   \item Have you related your theoretical results to the existing literature in social science?
%     \answerTODO{Answer}
%   \item Did you discuss the implications of your theoretical results for policy, practice, or further research in the social science domain?
%     \answerTODO{Answer}
% \end{enumerate}

% \item Additionally, if you are including theoretical proofs...
% \begin{enumerate}
%   \item Did you state the full set of assumptions of all theoretical results?
%     \answerTODO{Answer}
% 	\item Did you include complete proofs of all theoretical results?
%     \answerTODO{Answer}
% \end{enumerate}

\item Additionally, if you ran machine learning experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Yes, and code has been included as part of the supplemental material.} 
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Yes}
     \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{Yes}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Yes, and it has been added in the Limitations section}
     \item Do you justify how the proposed evaluation is sufficient and appropriate to the claims made? 
    \answerYes{Yes}
     \item Do you discuss what is ``the cost`` of misclassification and fault (in)tolerance?
    \answerYes{Yes}
  
\end{enumerate}

\item Additionally, if you are using existing assets (e.g., code, data, models) or curating/releasing new assets, \textbf{without compromising anonymity}...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{Yes}
  \item Did you mention the license of the assets?
    \answerNo{No, because the license of the assets are mentioned within the cited paper}
  \item Did you include any new assets in the supplemental material or as a URL?
    \answerYes{Yes}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{Yes}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{Yes}
\item If you are curating or releasing new datasets, did you discuss how you intend to make your datasets FAIR (see \citet{fair})?
\answerYes{Yes}
\item If you are curating or releasing new datasets, did you create a Datasheet for the Dataset (see \citet{gebru2021datasheets})? 
\answerNo{No, because it is a relatively simple dataset. But when we release it publicly such methods will be followed.}
\end{enumerate}

\item Additionally, if you used crowdsourcing or conducted research with human subjects, \textbf{without compromising anonymity}...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots?
    \answerYes{Yes, and it has been included in the appendix}
  \item Did you describe any potential participant risks, with mentions of Institutional Review Board (IRB) approvals?
    \answerYes{Yes}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerYes{Yes}
   \item Did you discuss how data is stored, shared, and deidentified?
   \answerNo{No, because we mentioned that it will be shared once the paper is accepted.}
\end{enumerate}
\end{enumerate}

==> sections/cne.tex <==
\section{Methodology}\label{sec:cne}
\subsection{Explainable Community Needs Extraction}\label{sec:llm_classification}
We define community needs extraction as the task of identifying need $\{n_1,n_2,n_3,..n_k\} \in N$ from the taxonomy of needs in each natural language conversation $c_i \in C_{needs}$ where $C_{needs}$ is the corpus of need-based conversations.  Vanilla CNE can be approached as an utterance-level classification~\cite{bakhtin_speech_nodate,evans_machine_2016}, but simply classifying community needs is not enough in-domain for producing urban community assessments - some rationalization is required. 

% However, NGOs require a certain amount of explainability and rationalization to perform needs assessments to categorize community needs. In this context, we define our method of explainable community needs extraction as a subgraph classification task with node attribution.  Graph Neural Networks (GNN) and GNN Explainers have been studied extensively to unlock and understand the opaque nature of classifications of deep learning models~\cite{ying_gnnexplainer_2019}.  


% We  as a subset of open information extraction (OIE) and graph representation learning will help increase the explainability of identifying community needs from conversations. 
% Such explainability can be extracted from the structural information present in conversations which can be represented as an OIE task of transforming natural language to a knowledge graph~\cite{angeli_leveraging_2015,mitchell_never-ending_2018}.
% It is this work on providing explainability that differs our work from other works in social media sentiment analysis and stance mining as discussed in Section~\ref{sec:related}.

Our overall approach for community needs extraction is shown in Figure~\ref{fig:architecture}. For each conversation $c_i \in C_{needs}$, we first perform zero-shot classification using the LLM prompt given in Figure~\ref{fig:prompt_class}.  Recent studies have shown that LLMs like ChatGPT outperform human annotators in labeling tasks \cite{gilardi_chatgpt_2023,huang_is_2023,wang_is_2023}. 
As a result, in this approach, given a conversation $c_i$ and pre-defined labels for needs $N\epsilon \{n_1, n_2, n_3,...\}$, we prompt a large language model to generate the label $y$. We experimented with multiple prompts, following best practices for prompt engineering prescribed for CSS~\cite{ziems_can_2023} , where we provided more fine-grained needs from the taxonomy as possible class labels. For example, we separated \textbf{E1: Basic Needs} into \textbf{Food and Nutrition} and \textbf{Health Care}, but the deconstruction of the need labels resulted in overwhelmingly more conversations being labeled as \textbf{E8: Not Applicable} indicating an increase in difficulty for an LLM to categorize said conversations. 

Each conversation $c_i \in C_{needs}$ was also transformed into an open information extraction (OIE) knowledge graph $(s,p,o) \in G_i$ where $s$ is the subject, $p$ is the predicate, and $o$ is the object. In the case of OIE all subjects, predicates, and objects are represented by ``words''~\cite{angeli_leveraging_2015,mitchell_never-ending_2018}.   For each community corpus of needs, $C_{needs}$ , we generate $G_i$ and $\{G_1,G_2,G_3,..G_n\} \in G$ where $G$ is the entire community knowledge graph. Each conversation is transformed by an LLM with the prompt given in Figure~\ref{fig:prompt_kg}. 




\begin{figure}
    \centering
    \includegraphics[scale=0.3]{images/architecture.png}
    \caption{Overall architecture of Explainable CNE}
    \label{fig:architecture}
\end{figure}


\begin{figure}[t]
    \centering
    \begin{simplebox}
        You are a knowledge graph creator.
        A knowledge graph contains entities and relations. Entities have properties ``name'' and ``type''. Relations have properties ``subject'', ``object'', and ``predicate''.
        For example, a knowledge graph can be written in JSON with the following structure:
        \begin{lstlisting}[language=json,firstnumber=1]
{
  "entities":[
    {
    "name":"",
    "type":""
    }
  ],
  "relations":[
    {
    "subject":"",
    "object":"",
    "predicate":""
    }
  ]
}
        \end{lstlisting}
    Convert the following text into a knowledge graph and return the answer as JSON:
\end{simplebox}
    \caption{Prompt for knowledge graph construction using LLMs}
    \label{fig:prompt_kg}
\end{figure}
Once the OIE knowledge graph $G_i$ for each conversation is built we generate feature embeddings for the subject and object in each OIE triple $(s_{ij},p_{ij},o_{ij})$ in $G_i$ using a BERT encoder~\cite{devlin_bert_2018}.  It is formulated as follows:
\begin{equation}
    f_{ij} = Encode(s_{ij}) \bigoplus Encode(o_{ij})
\end{equation}
where $i$ represents the subgraph index and $j$ represents the edge index in the graph $G_i$ , $\bigoplus$ represents concatenation, and $Encode$ returns a flattened vector representation of the outputs of the BERT encoder resulting in the aggregated feature vector $f_{ij}$ for each edge in $G_i$ represented by \textit{Aggregate} in the Figure~\ref{fig:architecture}. 

With the aggregated feature vector $f_{ij}$ containing the word embeddings and the structural information in $G_i$ and $G$, we utilize a two-layer feed-forward neural network using the $GraphSage$~\cite{hamilton_inductive_2018} layer for inductive learning,  a parametric ReLU activation function $PReLU$, and a final readout layer $GlobalMeanPool$, to take the average of the subgraph and node embeddings. We use cross-entropy loss comparing the label $y$ generated by zero-shot classification and the model output from the $Linear$ layer in Figure~\ref{fig:architecture}.

The subgraph classification model is then passed to a GNNExplainer~\cite{ying_gnnexplainer_2019}, which provides an explanation subgraph, where nodes and edges that did not contribute to the classification are masked. The basic formulation of generating an explanation is as follows.
Given the prediction $y = \phi(G_i,F_i, G)$, where $\phi$ is the CNE model, $G_i$ is the subgraph representation of the conversation, $G$ is the full knowledge graph representation of the corpus, and $F_i$ is the set of all features $f_{ij}$ generated by our aggregation function for subgraph $G_i$. 
GNNExplainer generates an explanation for $y$ as $G_s^M$ which is a subgraph of $G_i$ with nodes and edges masked out by mask $M$, while nodes and edges not masked out are most important for explaining $y$.
The results of this method are discussed in detail in Section~\ref{sec:evaluation}.

==> sections/evaluation.tex <==
\section{Evaluation and Discussion}\label{sec:evaluation}

\subsection{Zero-Shot CNE with LLMs}
In our experiments, we utilized our Reddit corpus to perform zero-shot text classification as outlined in Section~\ref{sec:llm_classification} classifying the community needs in the conversations using two popular and accessible large language models - Google's PaLM\cite{chowdhery_palm_2022} and OpenAI's ChatGPT. 
We have collected the results of previous urban community assessment performed in 2016 in the New York Area\cite{nyc_dycd_community_2022} as shown in Figure~\ref{fig:ground_truth_nyc_q3}. 
We compare and contrast the output of the two LLMs in addition to the results of the existing community assessment in the New York Area. The results of the survey are given in Figure~\ref{fig:ground_truth_nyc_q3}, as community residents were asked the question \textit{``What are the programs or services you believe are most needed in your community?''}. 
% In the absence of such ground truth, a noise audit can be performed to evaluate multiple decision-making systems.
% A noise audit, as described in \cite{kahneman_noise_2021}, is essentially an audit of outcome variability across multiple (competent) decision systems comparing and contrasting them to quantify results~\cite{rahwan_machine_2019}, and this approach has been previously used to evaluate offensive speech classifiers \cite{weerasooriya_vicarious_2023}. 


\begin{figure}[h]
    \centering
        \includegraphics[width=\linewidth]{images/nyc_ground_truth_q3.pdf}
    \caption{The results of a community needs assessment in the greater New York Area by the four communities. The y-axis represents ranking (0-7) with 7 being the highest ranked and 0 being the lowest. The x-axis represents each of the communities.}
        \label{fig:ground_truth_nyc_q3}
\end{figure}

We measured inter-annotator agreement between ChatGPT and PaLM with a mean Cohen's $\kappa$ of 0.15 across all communities - indicating low agreement between the two. However, this disagreement accounts for a significant portion of the conversations that were classified as \textbf{E8: Not Applicable}.
Within the conversations that were classified, Figure~\ref{fig:llm_text_classification_distribution} shows the proportion of conversations in our corpus classified to each of the needs. In both the LLMs and the survey results, we do see common trends. 
For example, conversations in all communities are primarily skewed towards \textbf{E1: Basic Needs}, and that is a significant portion of all communities according to the survey as well. 

In the subreddit \textit{r/nyc}, which may be considered a mixture of all the communities, after Basic Needs a majority of the conversations are focused on \textbf{E3: Employment} - a major concern in most communities except for Queens.
A difference between the survey results and our CNE result also indicates that there is more social media discourse about special population and support for senior citizens compared to concern in the survey sample - only the Bronx seem to have some need for special support compared to other boroughs according to the survey in Figure~\ref{fig:ground_truth_nyc_q3}. However, we see that is not the case in the results of our CNE in Figure~\ref{fig:llm_text_classification_distribution}. Another highlight is that a comparison between the need distribution in the mid-sized city of Rochester compared to a large one like New York City indicates disproportionate discussions about education and employment, while large city community conversations are primarily focused on support for special populations and families (Brooklyn and Bronx), along with basic needs.
\begin{figure}[h]
    \centering
    \quad
    \subfloat[PaLM]{\includegraphics[scale=0.25]{images/palm_text_classification_distribution.pdf}\label{subfig:palm_text_classification_distribution}}
    \quad
    \subfloat[ChatGPT]{\includegraphics[scale=0.25]{images/chatgpt_text_classification_distribution.pdf}    \label{subfig:chatgpt_text_classification_distribution}}
    \caption{Aggregated results of the community needs assessment performed in the four regions in New York City. the y-axis is the percentage of conversations, the x-axis is the subreddit}
    \label{fig:llm_text_classification_distribution}
\end{figure}




\begin{figure}[h]
\subfloat[LLM]{\includegraphics[width=\linewidth]{images/train_accuracy_by_llm.png}\label{fig:accuracy_llm}}
\quad
\subfloat[Subreddit]{\includegraphics[width=\linewidth]{images/train_accuracy_by_subreddit.png}\label{fig:accuracy_subreddit}}
\caption{Training accuracy for our explainable CNE model. We show the accuracy of each of the subreddit corpus and also by labels generated by each of the LLMs. All data points are the mean of 10 runs.}
\label{fig:accuracy}
\end{figure}

\begin{figure}[h]
    \centering
\subfloat[Post]{
\begin{chatbox1}
\textbf{Post:} Where to find non-profits that need in-kind donations from businesses for charity auctions/benefits?
I occasionally receive requests from non-profit organizations seeking in-kind donations of services for upcoming charity auctions. ... Does anyone know of a list or centralized website where I might find upcoming charity auctions that need donations?

\textbf{Comment:} Thanks! (I'm in NYC and work in education, so I'd be able to donate education-related services like test prep, college admission counseling, etc.)
Agreed. I'm on the exec board of a Park Slope PTA and, despite fantastic parental involvement and financial support, we are always looking for exactly this kind of thing.  ...  The former John Jay High School (7th Ave at 5th Street in Bklyn) houses 4 different public high schools now.  I suspect they'd love some guidance / test prep related services.
\end{chatbox1}
}
\quad
\subfloat[chatgpt]{\includegraphics[width=0.7\linewidth]{images/gpt_match.png}\label{subfig:llm_class_match_gpt}}

\subfloat[palm]{\includegraphics[width=0.7\linewidth]{images/palm_match.png}\label{subfig:llm_class_match_palm}}
    \caption{Example post from the subreddit \textit{r/Brooklyn}. Both LLMs labeled this post as E2: Education}
    \label{fig:llm_class_match}
\end{figure}

\begin{figure}[h]
    \centering
\begin{chatbox1}
\textbf{Post:}Moving back to NY(C) from Germany. What is reasonable pay to expect and/or ask for for relatively easy to obtain jobs. Please. 
... while I was there I generally asked for minimum wage, because I didn't know any better, so I don't have an idea of what's realistic, concerning salaries, wages, etc. I have some idea, since I've worked quite a lot, however some options are simply not currently available to me (e.g Working for UNICEF as face-to-face funds acquirer.)

\textbf{Comment:} Feel free to ask for info.
the stuff I need help with right now (and by right now, I mean I would literally pay \$40 an hour cash if someone was awake at 4 am reading this) is a welding project. simple art welds on 1/4" round with a MIG, nothing fancy or sexy or structural, and the appropriate cutting and cleaning.
\end{chatbox1}
\subfloat[chatgpt]{\includegraphics[width=0.7\linewidth]{images/gpt_mismatch.png}\label{subfig:llm_class_mismatch_gpt}}
\quad
\subfloat[palm]{\includegraphics[width=0.7\linewidth]{images/palm_mismatch.png}\label{subfig:llm_class_mismatch_palm}}
    \caption{Example post from the subreddit \textit{r/Brooklyn}. PaLM labeled E1: Basic Needs, ChatGPT labeled E3: Employment}
    \label{fig:llm_class_mismatch}
\end{figure}

\subsection{Explainable CNE}
We trained our explainable CNE architecture described in Section~\ref{sec:llm_classification} for each community separately with the following hyperparameters:~(1)~200 epochs,~(2)~Adam optimizer with learning rate $1e-4$,~(3)~batch size of 128,~(4)~maximum 256 tokens as output for the BERT encoder.
The training accuracy per epoch is shown in Figure~\ref{fig:accuracy}. In Figure~\ref{fig:accuracy_llm}, the training accuracy does not differ significantly when switching between the corpus labeled by each of the LLMs. 
However, in Figure~\ref{fig:accuracy_subreddit} the training accuracy is significantly lower for the subreddit \textit{r/nyc} compared to the other subreddits. A possible reason for this is that \textit{r/nyc} contains conversations regarding all the communities in the New York area, and such variance in the topic and needs is difficult for our model to accurately predict. 



Figure~\ref{fig:llm_class_match} shows an example text categorized as a discussion that was classified as \textbf{E2: Education} by both LLMs. While the post is a general query for where to donate - the comment is focused on where that donation is needed in the Brooklyn community. The knowledge subgraphs generated from this post in Figure~\ref{subfig:llm_class_match_gpt} and \ref{subfig:llm_class_match_gpt} displays how each of the LLMs deconstructs this text. We can see that ChatGPT retains significant amount of textual knowledge in its entities and relations, while PaLM reduces the scope to the bare minimum.  The explanation subgraph generated by our CNE masks the nodes and edges that did not contribute to the classification. In Figure~\ref{subfig:llm_class_match_gpt}, node \textit{I} is masked out.  Similarly, for Figure~\ref{subfig:llm_class_match_palm}, only the node \textit{Park Slope} is masked red indicating that it did not contribute to the classification i.e. locational information did not matter. 

In contrast, Figure~\ref{fig:llm_class_mismatch} shows an example of text categorized differently by the two LLMs - PaLM classifies the text as \textbf{E1: Basic Needs} while ChatGPT labels it \textbf{E3: Employment}. The difference in label can be explained by their explanation subgraphs. For ChatGPT, Figure~\ref{subfig:llm_class_mismatch_gpt} shows that most nodes were masked (i.e. they didn't contribute to the classification) except for the user name, location and the nodes \textit{wire management}, \textit{gas station jobs}, and \textit{CAD/CAM} with \textit{gas station jobs} significantly contributing to the employment label. In contrast, for PaLM in Figure~\ref{subfig:llm_class_mismatch_palm}  most nodes contributed to the classification resulting in the language model labeling the conversation as basic needs. However, if we read the conversation it is a difficult case as it can be classified as weakly basic needs (financial assistance) but strongly about employment. 

==> sections/limitations_old.tex <==
\section*{Limitations}
\paragraph{Resources}
Our explainable CNE models were trained on one NVIDIA A100 GPU with 40GB RAM, where the maximum training time was 20 minutes for a community with 2000 conversations for 200 epochs. While in the scale of large language model research that is a very modest time, even at this scale local NGOs (with scarce funding) may not have access to such high memory GPU. A more optimized training and inference approach will be required to implement this for such use cases.

\paragraph{Social}
We assumed that community needs can be classified given by assessments done in the past. 
But linguistically, further work is required into how people approach a conversation regarding needs and we need to deconstruct such an approach computationally to provide a more robust solution. Since our corpus in Reddit is already in the form of discussions such deconstruction was not necessary - but our future work will aim to broaden the modalities of conversations to other aspects such as focused-group discussions, one-on-one conversations, town hall meetings, etc.

\paragraph{Method}
Explanation subgraphs are not 100\% accurate and while we use a qualitative approach to show the usefulness of these explanations - human annotations to supplement our current community needs dataset would again increase the robustness and dependability of our proposed method. 
Our future work is working towards a multi-annotator labeled community needs gold dataset to supplement our current dataset. 
Furthermore, we use a shallow graph classification approach; a further study on deep graph neural networks and their explainability, leveraging the state-of-the-art chain of thought method on zero-shot classification explainability would provide a deeper understanding of the community needs conversation phenomena.
